Efficient and Effective Algorithms for A Family of Influence Maximization Problems with A Matroid Constraint

Influence maximization (IM) is a classic problem that aims to identify a small group of critical individuals, known as seeds, who can influence the largest number of users in a social network through word-of-mouth. This problem finds important applications including viral marketing, infection detection, and misinformation containment. The conventional IM problem is typically studied with the oversimplified goal of selecting a single seed set. Many real-world scenarios call for multiple sets of seeds, particularly on social media platforms where various viral marketing campaigns need different sets of seeds to propagate effectively. To this end, previous works have formulated various IM variants, central to which is the requirement of multiple seed sets, naturally modeled as a matroid constraint. However, the current best-known solutions for these variants either offer a weak $(1/2-\epsilon)$-approximation, or offer a $(1-1/e-\epsilon)$-approximation algorithm that is very expensive. We propose an efficient seed selection method called AMP, an algorithm with a $(1-1/e-\epsilon)$-approximation guarantee for this family of IM variants. To further improve efficiency, we also devise a fast implementation, called RAMP. We extensively evaluate the performance of our proposal against 6 competitors across 4 IM variants and on 7 real-world networks, demonstrating that our proposal outperforms all competitors in terms of result quality, running time, and memory usage. We have also deployed RAMP in a real industry strength application involving online gaming, where we show that our deployed solution significantly improves upon the baselines.

==> revision/cover-letter.tex <==

\renewcommand{\revise}[1]{{\color{blue} #1}}

\newenvironment{review}[1][]{\def\FrameCommand{\fboxsep=\FrameSep \fcolorbox{lightgray!30!white}{lightgray!30!white}} \color{black}\MakeFramed {\FrameRestore} {\vspace{-1mm}\noindent #1}}{\vspace{-2mm}\endMakeFramed}
\def\response{\noindent \textbf{Response}{: }}

\begin{titlepage}
    \begin{center}
       \textbf{\huge Cover Letter for PVLDB Volume 18 Submission \#169}
    \end{center}
\vspace{6mm}
\begin{Large}
{

 \section*{Executive Summary} 

Thanks for the opportunity for a revision! 
We also thank all reviewers for their valuable and constructive comments which have been helpful in improving the paper. The paper has been thoroughly revised based on the comments and shepherding guides, with all changes highlighted in \revise{blue}. Here is a summary of the changes made in the paper, in the order of their appearance:
\begin{itemize}
[topsep=2pt,itemsep=1pt,parsep=0pt,partopsep=0pt,leftmargin=11pt]
\item In Section \ref{sec:existing}, we have included the main idea of the reverse reachable (RR) set generation for the \ourproblem family and provided details for one instance, \mrim, as an example, in response to \textbf{R1W1}.

\item In Section \ref{sec:selection-overview}, we have included further discussions on potential applications of our proposed approaches, in response to \textbf{R3W1 \& R3D1}.

\item In Section \ref{sec:opim-main-idea}, we have corrected the notation $S^o$ to $S^o_1$ as suggested in \textbf{R1W2}.

\item In Section \ref{sec:exp}, as advised by \textbf{MR1 \& R2W1 \& R2D5}, we have included the Twitter-large dataset containing 41.7 million nodes and 1.5 billion edges. Specifically, we evaluated the performance of the algorithms on Twitter-large in terms of solution quality, running time, and memory footprints, and reported the corresponding results in Figures \ref{fig:rm-spread}-\ref{fig:scale-all-memory}. We have also updated the dataset statistics in Table \ref{tab:dataset}, as suggested by \textbf{MR3 \& R1W3}. Furthermore, in response to \textbf{MR2 \& R2W2}, we have reported the memory usage of scalable implementations in Figure \ref{fig:scale-all-memory} of the revised manuscript. 

\eat{\item In Section \ref{sec:exp-performance}, due to space constraints, we have deferred experiments regarding the running times of scalable implementations on small datasets to a technical report. We only report results on the largest dataset, where the baseline algorithm with $\epsilon=0.5$ can terminate within 72 hours, as shown in Figure \ref{fig:scale-all-time}.}

\item We note that incorporating the reviewer comments has resulted in the addition of new figures and references,\eat{$\langle$figures, tables, and references$\rangle$, [UPDATE THIS AS APPROPRIATE.]} leading to changes in the numbers. Besides, in order to make room for the new added material, we have had to remove two figures from the revised version. To demonstrate maximum scalability, we retain figures for the largest datasets in each \ourproblem instance on which the baseline algorithm can terminate within 72 hours when $\epsilon=0.5$. For smaller datasets, we defer the corresponding figures to a technical report. Nevertheless, we note that results in the removed figures show trends similar to those in other figures that are included in the paper. For example, Figure \ref{fig:scale-all-time}(a) of the revised version closely resembles Figure 7(d) of the submitted version, where \ouralgo outperforms \rma in terms of running time by about $10\times$ while guaranteeing the same approximation. In addition, Figure \ref{fig:scale-all-time}(b) of the revised version is similar to Figure 8(a) of the submitted version, where \ouralgo is at least three orders of magnitudes faster than \rma.\eat{$\langle$ We took care to make sure that results in the removed figures show trends similar to those in other figures that are included in the paper. For example, ...$\rangle$ [FILL IN THE DETAILS AND JUSTIFICATION HERE].} Below, we provide a mapping between numbers in the submitted version of the paper and the revised version for convenience (see Table \ref{tab:old-fig-pos}).

\renewcommand{\thetable}{A}
\begin{table}[h]
\centering
\caption{Mapping between numbers in the submitted version of the paper and the revised version.}\label{tab:old-fig-pos}
\vspace{-3mm}
\renewcommand{\arraystretch}{1.2}
\begin{small}
\begin{tabular}{ccccc}
\toprule
{\bf Submitted version} & Figure 8(b) & Figure 8(c) & Figure 7 and Figure 8(a) & Citations [54-56] \\ 
\midrule 
{\bf Revised version} & Figure \ref{fig:scale-all-time}(b) & Figure \ref{fig:scale-all-time}(c) & deferred to a technical report & Citations [56-58] \\ 
\bottomrule
\end{tabular}
\end{small}
\end{table}

\item We use letters for referring to figures, tables, and references in the cover letter and use numbers to refer to those in the paper. E.g., Table A, paper [b], and Figure C refer to those in the cover letter. 
Table \ref{tab:fig-pos} provides a link between letters in the cover letter and their corresponding numbers in the paper. Please note that Figures \ref{fig:rm-memory}(a)-(f) and Figure \ref{fig:other-memory}(a) in this cover letter have been deferred to a technical report.

\renewcommand{\thetable}{B}
\begin{table}[h]
\centering
\caption{Positions of the new figures in the revised manuscript.}\label{tab:fig-pos}
\vspace{-3mm}
\renewcommand{\arraystretch}{1.2}
\begin{small}
\begin{tabular}{cccccccccc}
\toprule
{\bf Letter} & Figure \ref{fig:result-tw}(a) & Figure \ref{fig:result-tw}(b) & Figure \ref{fig:result-tw}(c) &Figure \ref{fig:result-tw}(d) & Figure \ref{fig:tw-rm-time} & Figure \ref{fig:tw-rm-scale-time} & Figure \ref{fig:rm-memory}(g) & Figure \ref{fig:other-memory}(b) & Figure \ref{fig:other-memory}(c) \\ 
\midrule 
{\bf Number} & Figure \ref{fig:rm-spread}(g) & Figure \ref{fig:mrim-spread}(g) & Figure \ref{fig:advim-spread}(g) & Figure \ref{fig:im-spread}(g) & Figure \ref{fig:rm-time}(g) & Figure \ref{fig:scale-all-time}(a) & Figure \ref{fig:scale-all-memory}(a) & Figure \ref{fig:scale-all-memory}(b) & Figure \ref{fig:scale-all-memory}(c) \\
\bottomrule
\end{tabular}
\end{small}
\end{table}
\end{itemize}

}
\end{Large}

\end{titlepage}

\begin{titlepage}


\section*{Shepherding from Meta-Reviewer}
\vspace{-1mm}
{
\Large
\begin{review}
{\bf MR1.} The datasets used in the experimental analysis are very small with a maximum of 4.8M nodes and 69 million edges which is quite small compared to real world graphs with billions of edges. Please report the results of experiments with larger data sets.
\end{review}\vspace{-1mm}

\response As suggested, we have included the Twitter-large dataset consisting of 41.7 million nodes and 1.5 billion edges, and reported the experimental results in terms of result quality, running time, and resource utilization. Please refer also to our response to {\bf R2W1 \& R2D5}.

\begin{review}
{\bf MR2.} Describe the resource utilization of the proposed approach, e.g., space consumption.
\end{review}\vspace{-1mm}

\response We have compared all scalable solutions in terms of the memory footprint. In a nutshell, the results demonstrate the  superiority of our approach w.r.t. resource utilization. Please refer to our response to {\bf R2W2} for details.

\begin{review}
{\bf MR3.} The types of datasets used are not stated. Specify the type of social network for each dataset.
\end{review}\vspace{-1mm}

\response We have summarized the types of datasets in Table \ref{tab:dataset-revised}. Please refer to our response to {\bf R1W3}.

}  


\section*{Reviewer 1}
\vspace{-1mm}
{
\Large
\begin{review}
{\bf R1W1.} In Section 2.4, the authors mention that the strategy of RR set construction is personalized to the IM-GM instance. The authors should clarify the procedure for different instances.
\end{review}\vspace{-1mm}

\response 
We apologize for omitting the details owing to lack of space. To explain, each \ourproblem instance involves a specific diffusion model and a corresponding reverse diffusion process. Take the vanilla \im as an example. The reverse diffusion process of the Independent Cascade model is a stochastic breadth-first search starting from $v_i$. For each visited $v_a$, it explores each in-neighbor $v_b \in N^{in}_a$ with probability $p_{b,a}$.
Regarding the \ourproblem instances used in our work, we follow the original works and recap below the generation procedure of an RR set $R$ for each \ourproblem instance.
\begin{itemize}[topsep=2pt,itemsep=1pt,parsep=0pt,partopsep=0pt,leftmargin=11pt]
    \item \textit{\im}: We first select a node $v_i\in V$ uniformly at random, and then simulate a reverse diffusion process in $G$ starting from $v_i$. We let $R$ be the set of all examined nodes.
    \item \textit{\mrim}: We first randomly select a node $v_i\in V$ uniformly, and then independently simulate $T$ reverse diffusion processes starting from $v_i$, denoting the set of examined nodes in each process as $R'_1, \dots, R'_T$. We finally let $R \gets R'_1\times\{1\}\cup\dots\cup R'_T\times\{T\}$.
    \item \textit{\rim}: We first randomly select a node $v_i\in V$ uniformly, and a campaign index $j\in [T]$ w.p. $\frac{\alpha_j}{\sum_{j\in [T]}\alpha_j}$. We simulate a reverse diffusion process starting from $v_i$, denoting the set of examined nodes as $R'$. Then, we let $R \gets R'\times\{j\}$.
    \item \textit{\advim}: We first select a node $v_i\in V\backslash A$ uniformly at random, and then simulate the reverse diffusion process from $v_i$ and include the examined nodes into $R$. If $R\cap A=\emptyset$, we clear $R$ and repeat the process until $R\cap A\neq\emptyset$.
\end{itemize}
In the revised manuscript, we have included the main idea of RR set generation and the detail for \mrim in Section \ref{sec:existing}. Due to space constraints, we have deferred complete details for the rest of the instances to a technical report. We hope this is acceptable. 


\begin{review}
{\bf R1W2.} The notation of $S^o$ in Section 5.1 seems confused with those in Section 4. If $S^o$ represents the optimal coverage solution on a different set of RR sets $\mathcal{R}_1$(but not $\mathcal{R}$), it would be clearer to use $S^o_1$ or other subscript instead.
\end{review}
\vspace{-1mm}

\response Thanks for pointing out the potential confusion caused by our original notation. We have corrected it as suggested.
}

\end{titlepage}

\begin{titlepage}

{
\Large
\begin{review}
{\bf R1W3.} The types of datasets used are not stated in this paper. It would be great if adding a statement specifying the type of social network for each dataset.
\end{review}
\vspace{-1mm}

\response As suggested, we have included the type of the underlying social network for each dataset (see Table \ref{tab:dataset-revised}) and updated Table \ref{tab:dataset} in the revised manuscript.
}

\renewcommand{\thetable}{C}
\begin{table}[h]
\centering
\caption{Dataset statistics. ($K=10^3, M=10^6, B=10^9$)}\label{tab:dataset-revised}
\vspace{-3mm}
\renewcommand{\arraystretch}{1.2}
\begin{small}
\begin{tabular}{ccccc}
\toprule
\textbf{Name}     & \textbf{\#nodes} & \textbf{\#edges} & {\textbf{Type}} & {\textbf{Avg. degree}} \\ 
% \textbf{Name}     & Facebook & Wiki & Twitter & Google+ & Pokec & LiveJournal \\ 
\midrule 
Facebook & $4.0K$ & $176.4K$ & {friendship} & {$43.6$}\\
Wiki & $7.1K$ & $103.6K$ & {who-votes-on-whom} & {$14.5$}\\
Twitter & $81.3K$ & $1.7M$ & {who-follows-whom} & {$21.7$}\\
Google+ & $107.6K$ & $13.7M$ & {who-follows-whom} & {$283.3$}\\
Pokec & $1.6M$ & $30.6M$ & {friendship} & {$18.7$}\\
LiveJournal & $4.8M$ & $69.0M$ & {friendship} & {$14.2$}\\
Twitter-large & $41.7M$ & $1.5B$ & {who-follows-whom} & {$35.2$}\\
\bottomrule
\end{tabular}
\end{small}
\end{table}

\section*{Reviewer 2}
\vspace{-1mm}
{
\Large
\begin{review}
{\bf R2W1 \& R2D5.} The datasets used in the experimental analysis are very small with a maximum of 4.8M nodes and 69 million edges which is quite small compared to real world graphs with billions of edges.
\end{review}\vspace{-1mm}

\response As suggested, we have included the Twitter-large dataset, which consists of 41.7 million nodes and 1.5 billion edges, making it the largest dataset ever used in instances \rim, \mrim, and \advim. The performance of each solution on this dataset is summarized in the following.
\begin{itemize}[topsep=2pt,itemsep=1pt,parsep=0pt,partopsep=0pt,leftmargin=11pt]
\item First, we have evaluated the result quality of each element selection algorithm in terms of related objective functions. As reported in Figure~\ref{fig:result-tw}, our \cseedselect or \cseedselectp outperforms all competitors by up to 49.7\% in \rim, 110.7\% in \mrim, 205.8\% in \advim, and 146.9\% in \im.
\item Second, we have evaluated the running time of all element selection algorithms and scalable implementations. As in the submitted manuscript, we only report the results on the \rim problem. The reasons are two-fold. First, the running times of element selection algorithms for other \ourproblem instances show similar trends. Second, the state-of-the-art scalable algorithms for \mrim and \advim cannot terminate on Twitter-large within 72 hours. \eat{[SOMEWHERE YOU NEED TO SAY WHAT IS REASONABLE, I.E., WHEN YOU CUT OFF.]} As reported in Figure~\ref{fig:tw-rm-time}, the running time of element selection algorithms shows a similar trend to those in smaller datasets, where \cseedselectp (with $\epsilon=0.5$) is the second most efficient algorithm. Additionally, Figure \ref{fig:tw-rm-scale-time} shows that \ouralgo is at least an order of magnitude faster than \rma. Notably, \ouralgo ends within 66 hours when $\epsilon=0.3$, whereas \rma only returns results for $\epsilon\geq 0.4$ and \textit{fails to terminate even after 7 days when $\epsilon=0.3$.} 
\item We have also evaluated the memory usage of all solutions.  We defer this discussion to our response to {\bf R2W2}. 
\end{itemize}
In the revised manuscript, we have included Figures \ref{fig:result-tw}-\ref{fig:tw-rm-scale-time} among Figures \ref{fig:rm-spread}-\ref{fig:scale-all-time}. The corresponding positions where they have been inserted into the paper can be found in Table \ref{tab:fig-pos}.
\eat{[MIGHT WANT TO SAY WHAT FIG. A-C CORRESPOND TO AMONG FIG. 2-7.]}
}

\input{revision/twitter-large}

\end{titlepage}

\begin{titlepage}

\input{revision/twitter-scale-large}


{
\Large

    \begin{review}
{\bf R2W2.} The only metric used for comparing efficiency, a major contribution of the paper is running time. There are no metrics that describe the resource utilization of the proposed approach.
\end{review}\vspace{-1mm}

\response Thank you for this great suggestion. Following your suggestion, we have measured the resource utilization using memory usage, and reported the memory usage of each scalable implementation for each mentioned \ourproblem instance in Figures \ref{fig:rm-memory}-\ref{fig:other-memory}. Please note that the reported numbers correspond to peak memory consumption of each scalable implementation. 

\input{revision/fig-memory}
\input{revision/fig-memory-others}

}
\end{titlepage}

\begin{titlepage}

{
\Large

As shown, the memory usage of each algorithm is roughly proportional to its running time reported in Figures 7-8 of the submitted manuscript. Most notably, the memory occupancy of \ouralgo is consistently lower than that of \rma, \naimm, and \advimm due to the smaller number of sampled RR sets. Specifically, the memory footprint of \ouralgo in \mrim is at least an order of magnitude lower than \naimm on Facebook and Wiki. Note that, \ouralgo or \rma uses a memory footprint of 102GB on Twitter-large when $\epsilon \geq 0.4$. Of this, 62GB is allocated for storing the dataset (with half for the original graph and half for the reversed graph, on which the RR sets are generated), while the remaining 40 GB memory ($\sim$39\%) is used for storing the sampled RR sets.

% Notice that this tendency is less pronounced on Twitter-large in \rim, as shown in Figure \ref{fig:rm-memory}(g), because storing the dataset requires a larger proportion of space than the actual size of generated RR sets, although the time for generating an RR set is substantial.
In the revised manuscript, we have included Figure \ref{fig:rm-memory}(g), Figure \ref{fig:other-memory}(b), and Figure \ref{fig:other-memory}(c) as Figure \ref{fig:scale-all-memory} in Section \ref{sec:exp}. Due to limited space, we have deferred other results to a technical report.
We hope this is acceptable.


\begin{review}
{\bf R2W3.} Solutions for a distributed setting are not considered and left as future work.
\end{review}\vspace{-1mm}

\response Thank you for pointing out this issue. We would like to clarify that implementing our solutions in a distributed fashion is non-trivial. For the element selection subroutine \cseedselect, it involves $1/\epsilon-1$ more iterations compared to \mgreedy, resulting in higher communication costs among different machines. For the RR set generation, although Tang et al.~\ref{ref:tang2022} has studied its distributed setting for the \im problem, it remains unclear how to extend these approaches to other \ourproblem instances and whether each instance requires a personalized algorithm implementation. In view of these challenges, we leave designing new solutions for the distributed setting as future work.
}


    \section*{Reviewer 3}
\vspace{-1mm}
{
\Large
\begin{review}
{\bf R3W1 \& R3D1.} While the authors discuss the potential application of the problem studied in this paper and provide multiple citations, I see the application scope as somewhat limited.
\end{review}\vspace{-1mm}

\response Thank you for pointing out this issue. We would like to clarify that, besides various instances in the \ourproblem family as discussed in our paper, our proposed approaches \cseedselect and \ouralgo have potential applicability in \im scenarios that leverage the multilinear extension. There are practical problem settings of \im variants which can directly benefit from this. For example, consider \im variants constrained to user groups~\ref{ref:udwani2018} and \im with group fairness~\ref{ref:tsang2019}. We can enhance the efficiency of solutions for these problems by replacing the traditional multilinear extension format with the RR sets format and redesigning the methodology accordingly.
We have included the related discussions in Section~\ref{sec:selection-overview}.

}

\vspace{3cm}

\section*{References}

\begin{enumerate}[label={[\alph*]}, leftmargin=*]
\item Jing Tang, Yuqing Zhu, Xueyan Tang, and Kai Han. 2022. Distributed Influence Maximization for Large-Scale Online Social Networks. In ICDE. 81–95.\label{ref:tang2022}
\item Rajan Udwani. 2018. Multi-Objective Maximization of Monotone Submodular Functions with Cardinality Constraint. In NeurIPS. 9513–9524.\label{ref:udwani2018}
\item Alan Tsang, Bryan Wilder, Eric Rice, Milind Tambe, and Yair Zick. 2019. Group-Fairness in Influence Maximization. In IJCAI. 5997–6005.\label{ref:tsang2019}
\end{enumerate}

\end{titlepage}

\setcounter{table}{0}
\setcounter{figure}{0}

\clearpage

==> revision/fig-memory-others.tex <==
\vspace{-4mm}
\renewcommand{\thefigure}{E}
\begin{figure}[h]
\centering
% \vspace{-2.5mm}
\begin{tikzpicture}
    \begin{customlegend}[legend columns=3,
        legend entries={\ouralgo, \naimm, \advimm
        }
        ,
        legend style={at={(0.45,1.05)},anchor=north,draw=none,font=\footnotesize,column sep=0.1cm}]
    \addlegendimage{line width=0.25mm,mark size=2pt,mark=triangle,color=Red}
    \addlegendimage{line width=0.25mm,mark size=2pt,mark=o, color=LightBlue}
    \addlegendimage{line width=0.25mm,mark size=2pt,mark=square, color=Green}
    \end{customlegend}
    %  \begin{customlegend}[legend columns=6,
    %     legend entries={},
    %     legend style={at={(0.45,0.7)},anchor=north,draw=none,font=\footnotesize,column sep=0.1cm}]
 
    % \end{customlegend}
\end{tikzpicture}
\vspace{-2mm}
\\[-\lineskip]
\hspace{-3mm}\subfloat[\mrim, Facebook]{
\begin{tikzpicture}[scale=1]
    \begin{axis}[
        height=(\columnwidth/1.95)/2.8,
        width=(\columnwidth/1.95)/2.25,
        ylabel={memory usage (MB)},
        xlabel={approx. guarantee},
        xmin=0, xmax=0.6,
        ymin=10000, ymax=10000000,
        xtick={0,0.2, 0.4,0.6},
        xticklabel style = {font=\footnotesize},
        xticklabels={0,0.2, 0.4,0.6},
        ytick={10000, 100000, 1000000, 10000000},
        yticklabels={$10^2$, $10^3$, $10^4$, $10^5$},
        ymode=log,
        log basis y={10},
        every axis y label/.style={at={(current axis.north west)},right=10.3mm,above=0mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
        every axis x label/.style={at={(current axis.south)},right=0mm,above=-7mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
    ]


    \addplot[line width=0.2mm,mark size=2.0pt,mark=o, color=LightBlue]
        plot coordinates { % CR-MRIMM
        (0, 226640)
        (0.1, 321736)
        (0.2, 503772)
        (0.3, 987056)
        (0.4, 3317692)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=triangle,color=Red]
        plot coordinates { % ours
        (0.13212+0, 48692)
        (0.13212+0.1, 64484)
        (0.13212+0.2, 65808)
        (0.13212+0.3, 66952)
        (0.13212+0.4, 79532)
    };
    \end{axis}
\end{tikzpicture}\vspace{1mm}\hspace{1mm}%
}%
\hspace{-4mm}\subfloat[\mrim, Wiki]{
\begin{tikzpicture}[scale=1]
    \begin{axis}[
        height=(\columnwidth/1.95)/2.8,
        width=(\columnwidth/1.95)/2.25,
        ylabel={memory usage (MB)},
        xlabel={approx. guarantee},
        xmin=0, xmax=0.6,
        ymin=60000, ymax=10000000,
        xtick={0,0.2, 0.4,0.6},
        xticklabel style = {font=\footnotesize},
        xticklabels={0,0.2, 0.4,0.6},
        ytick={100000, 1000000, 10000000},
        yticklabels={$10^3$, $10^4$, $10^5$},
        ymode=log,
        log basis y={10},
        every axis y label/.style={at={(current axis.north west)},right=10.3mm,above=0mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
        every axis x label/.style={at={(current axis.south)},right=0mm,above=-7mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
    ]


    \addplot[line width=0.2mm,mark size=2.0pt,mark=o, color=LightBlue]
        plot coordinates { % CR-MRIMM
        (0, 320772)
        (0.1, 457388)
        (0.2, 729404)
        (0.3, 1473896)
        (0.4, 4963396)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=triangle,color=Red]
        plot coordinates { % ours
        (0.13212+0, 96132)
        (0.13212+0.1, 98240)
        (0.13212+0.2, 204908)
        (0.13212+0.3, 213112)
        (0.13212+0.4, 356000)
    };
    \end{axis}
\end{tikzpicture}\vspace{1mm}\hspace{1mm}%
}%
\hspace{-4mm}\subfloat[\advim, Wiki]{
\begin{tikzpicture}[scale=1]
    \begin{axis}[
        height=(\columnwidth/1.95)/2.8,
        width=(\columnwidth/1.95)/2.25,
        ylabel={memory usage (MB)},
        xlabel={approx. guarantee},
        xmin=0, xmax=0.6,
        ymin=10000, ymax=1000000,
        xtick={0,0.2, 0.4,0.6},
        xticklabel style = {font=\footnotesize},
        xticklabels={0,0.2, 0.4,0.6},
        ytick={10000, 100000, 1000000},
        yticklabels={$10^1$, $10^2$, $10^3$},
        ymode=log,
        log basis y={10},
        every axis y label/.style={at={(current axis.north west)},right=10.3mm,above=0mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
        every axis x label/.style={at={(current axis.south)},right=0mm,above=-7mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
    ]


    \addplot[line width=0.2mm,mark size=2.0pt,mark=square, color=Green]
        plot coordinates { % AAIMM
        (0, 29712)
        (0.1, 36344)
        (0.2, 49204)
        (0.3, 85568)
        (0.4, 272916)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=triangle,color=Red]
        plot coordinates { % ours
        (0.13212+0, 19044)
        (0.13212+0.1, 19096)
        (0.13212+0.2, 22820)
        (0.13212+0.3, 22912)
        (0.13212+0.4, 23164)
    };
    \end{axis}
\end{tikzpicture}\vspace{1mm}\hspace{1mm}%
}%
\vspace{-3mm}
\caption{Memory usage in \mrim and \advim. Experiments that exceed 72 hours have been excluded.} \label{fig:other-memory}
\vspace{-3mm}
\end{figure}

==> revision/fig-memory.tex <==
\vspace{-3mm}
\renewcommand{\thefigure}{D}
\begin{figure}[h]
\centering
% \vspace{-2.5mm}
\begin{tikzpicture}
    \begin{customlegend}[legend columns=2,
        legend entries={\ouralgo, \rma
        }
        ,
        legend style={at={(0.45,1.05)},anchor=north,draw=none,font=\footnotesize,column sep=0.1cm}]
    \addlegendimage{line width=0.25mm,mark size=2pt,mark=triangle,color=Red}
    \addlegendimage{line width=0.25mm,mark size=2pt,mark=pentagon,color=Pink}
    \end{customlegend}
    %  \begin{customlegend}[legend columns=6,
    %     legend entries={},
    %     legend style={at={(0.45,0.7)},anchor=north,draw=none,font=\footnotesize,column sep=0.1cm}]
 
    % \end{customlegend}
\end{tikzpicture}
\vspace{-2mm}
\\[-\lineskip]
\hspace{-4mm}\subfloat[{Facebook}]{
\begin{tikzpicture}[scale=1]
    \begin{axis}[
        height=(\columnwidth/1.95)/2.8,
        width=(\columnwidth/1.95)/2.25,
        ylabel={memory usage (MB)},
        xlabel={approx. guarantee},
        xmin=0, xmax=0.6,
        ymin=10000, ymax=160000,
        xtick={0,0.2, 0.4,0.6},
        xticklabel style = {font=\footnotesize},
        xticklabels={0,0.2, 0.4,0.6},
        ytick={10000,100000},
        yticklabels={$10^1$, $10^2$},
        ymode=log,
        log basis y={10},
        every axis y label/.style={at={(current axis.north west)},right=10.3mm,above=0mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
        every axis x label/.style={at={(current axis.south)},right=0mm,above=-7mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
    ]


    \addplot[line width=0.2mm,mark size=2.0pt,mark=pentagon,color=Pink]
        plot coordinates { 
        (0,16596)
        (0.1,17132)
        (0.2,23624)
        (0.3,44636)
        (0.4,128328)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=triangle,color=Red]
        plot coordinates { % ours
        (0.13212+0, 16296)
        (0.13212+0.1, 16180)
        (0.13212+0.2, 19572)
        (0.13212+0.3, 33360)
        (0.13212+0.4, 54736)
    };
    
    \end{axis}
\end{tikzpicture}\vspace{1mm}\hspace{1mm}%
}%
\hspace{-4mm}\subfloat[{Wiki}]{
\begin{tikzpicture}[scale=1]
    \begin{axis}[
        height=(\columnwidth/1.95)/2.8,
        width=(\columnwidth/1.95)/2.25,
        ylabel={memory usage (MB)},
        xlabel={approx. guarantee},
        xmin=0, xmax=0.6,
        ymin=10000, ymax=1000000,
        xtick={0,0.2, 0.4,0.6},
        xticklabel style = {font=\footnotesize},
        xticklabels={0,0.2, 0.4,0.6},
        ytick={10000,100000,1000000},
        yticklabels={$10^1$, $10^2$, $10^3$},
        ymode=log,
        log basis y={10},
        every axis y label/.style={at={(current axis.north west)},right=10.3mm,above=0mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
        every axis x label/.style={at={(current axis.south)},right=0mm,above=-7mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
    ]


    \addplot[line width=0.2mm,mark size=2.0pt,mark=pentagon,color=Pink]
        plot coordinates { 
        (0,16288)
        (0.1,19260)
        (0.2,28916)
        (0.3,111392)
        (0.4,395068)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=triangle,color=Red]
        plot coordinates { % ours
        (0.13212+0,16068)
        (0.13212+0.1,21208)
        (0.13212+0.2,28956)
        (0.13212+0.3,45032)
        (0.13212+0.4,81008)
    };
    
    \end{axis}
\end{tikzpicture}\vspace{1mm}\hspace{1mm}%
}%
\hspace{-4mm}\subfloat[{Twitter}]{
\begin{tikzpicture}[scale=1]
    \begin{axis}[
        height=(\columnwidth/1.95)/2.8,
        width=(\columnwidth/1.95)/2.25,
        ylabel={memory usage (MB)},
        xlabel={approx. guarantee},
        xmin=0, xmax=0.6,
        ymin=100000, ymax=3120000,
        xtick={0,0.2, 0.4,0.6},
        xticklabel style = {font=\footnotesize},
        xticklabels={0,0.2, 0.4,0.6},
        ytick={100000,1000000},
        yticklabels={$10^2$, $10^3$},
        ymode=log,
        log basis y={10},
        every axis y label/.style={at={(current axis.north west)},right=10.3mm,above=0mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
        every axis x label/.style={at={(current axis.south)},right=0mm,above=-7mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
    ]


    \addplot[line width=0.2mm,mark size=2.0pt,mark=pentagon,color=Pink]
        plot coordinates { 
        (0,143088)
        (0.1,158984)
        (0.2,240212)
        (0.3,430168)
        (0.4,2122760)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=triangle,color=Red]
        plot coordinates { % ours
        (0.13212+0,154512)
        (0.13212+0.1,159160)
        (0.13212+0.2,173436)
        (0.13212+0.3,305628)
        (0.13212+0.4,790584)
    };
    
    \end{axis}
\end{tikzpicture}\vspace{1mm}\hspace{1mm}%
}%
\hspace{-4mm}\subfloat[{Google+}]{
\begin{tikzpicture}[scale=1]
    \begin{axis}[
        height=(\columnwidth/1.95)/2.8,
        width=(\columnwidth/1.95)/2.25,
        ylabel={memory usage (MB)},
        xlabel={approx. guarantee},
        xmin=0, xmax=0.6,
        ymin=1000000, ymax=10000000,
        xtick={0,0.2, 0.4,0.6},
        xticklabel style = {font=\footnotesize},
        xticklabels={0,0.2, 0.4,0.6},
        ytick={1000000,10000000},
        yticklabels={$10^3$, $10^4$},
        ymode=log,
        log basis y={10},
        every axis y label/.style={at={(current axis.north west)},right=10.3mm,above=0mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
        every axis x label/.style={at={(current axis.south)},right=0mm,above=-7mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
    ]


    \addplot[line width=0.2mm,mark size=2.0pt,mark=pentagon,color=Pink]
        plot coordinates { 
        (0,1265028)
        (0.1,1299956)
        (0.2,1397500)
        (0.3,2246180)
        (0.4,5038128)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=triangle,color=Red]
        plot coordinates { % ours
        (0.13212+0,1271964)
        (0.13212+0.1,1271916)
        (0.13212+0.2,1289132)
        (0.13212+0.3,1832272)
        (0.13212+0.4,2510488)
    };
    
    \end{axis}
\end{tikzpicture}\vspace{1mm}\hspace{1mm}%
}%
\\
\hspace{-4mm}\subfloat[{Pokec}]{
\begin{tikzpicture}[scale=1]
    \begin{axis}[
        height=(\columnwidth/1.95)/2.8,
        width=(\columnwidth/1.95)/2.25,
        ylabel={memory usage (MB)},
        xlabel={approx. guarantee},
        xmin=0, xmax=0.6,
        ymin=1000000, ymax=100000000,
        xtick={0,0.2, 0.4,0.6},
        xticklabel style = {font=\footnotesize},
        xticklabels={0,0.2, 0.4,0.6},
        ytick={1000000,10000000,100000000},
        yticklabels={$10^3$, $10^4$, $10^5$},
        ymode=log,
        log basis y={10},
        every axis y label/.style={at={(current axis.north west)},right=10.3mm,above=0mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
        every axis x label/.style={at={(current axis.south)},right=0mm,above=-7mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
    ]


    \addplot[line width=0.2mm,mark size=2.0pt,mark=pentagon,color=Pink]
        plot coordinates { 
        (0,2549844)
        (0.1,2741108)
        (0.2,4297512)
        (0.3,14855112)
        (0.4,50378040)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=triangle,color=Red]
        plot coordinates { % ours
        (0.13212+0,2592460)
        (0.13212+0.1,2621324)
        (0.13212+0.2,2877532)
        (0.13212+0.3,9599256)
        (0.13212+0.4,17792136)
    };
    
    \end{axis}
\end{tikzpicture}\vspace{1mm}\hspace{1mm}%
}%
\hspace{-4mm}\subfloat[{LiveJournal}]{
\begin{tikzpicture}[scale=1]
    \begin{axis}[
        height=(\columnwidth/1.95)/2.8,
        width=(\columnwidth/1.95)/2.25,
        ylabel={memory usage (MB)},
        xlabel={approx. guarantee},
        xmin=0, xmax=0.6,
        ymin=3160000, ymax=312000000,
        xtick={0,0.2, 0.4,0.6},
        xticklabel style = {font=\footnotesize},
        xticklabels={0,0.2, 0.4,0.6},
        ytick={10000000, 100000000},
        yticklabels={$10^4$, $10^5$},
        ymode=log,
        log basis y={10},
        every axis y label/.style={at={(current axis.north west)},right=10.3mm,above=0mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
        every axis x label/.style={at={(current axis.south)},right=0mm,above=-7mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
    ]


    \addplot[line width=0.2mm,mark size=2.0pt,mark=pentagon,color=Pink]
        plot coordinates { 
        (0,6596336)
        (0.1,7016296)
        (0.2,11440888)
        (0.3,23991124)
        (0.4,137534900)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=triangle,color=Red]
        plot coordinates { % ours
        (0.13212+0,6620992)
        (0.13212+0.1,6696448)
        (0.13212+0.2,9220792)
        (0.13212+0.3,26044400)
        (0.13212+0.4,48664084)
    };
    
    \end{axis}
\end{tikzpicture}\vspace{1mm}\hspace{1mm}%
}%
\hspace{-4mm}\subfloat[{Twitter-large}]{
\begin{tikzpicture}[scale=1]
    \begin{axis}[
        height=(\columnwidth/1.95)/2.8,
        width=(\columnwidth/1.95)/2.25,
        ylabel={memory usage (GB)},
        xlabel={approx. guarantee},
        xmin=0, xmax=0.6,
        ymin=100000000, ymax=120000000,
        xtick={0,0.2, 0.4,0.6},
        xticklabel style = {font=\footnotesize},
        xticklabels={0,0.2, 0.4,0.6},
        ytick={100000000, 120000000},
        yticklabels={100,120},
        ymode=log,
        log basis y={10},
        every axis y label/.style={at={(current axis.north west)},right=10.3mm,above=0mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
        every axis x label/.style={at={(current axis.south)},right=0mm,above=-7mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
    ]


    \addplot[line width=0.2mm,mark size=2.0pt,mark=pentagon,color=Pink]
        plot coordinates { 
        (0,101925836)
        (0.1,102007436)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=triangle,color=Red]
        plot coordinates { % ours
        (0.13212+0, 101920900)
        (0.13212+0.1,101939008)
        (0.13212+0.2,116192608)
    };
    
    \end{axis}
\end{tikzpicture}\vspace{1mm}\hspace{1mm}%
}%
\vspace{-3mm}
\caption{Memory usage in \rim. Experiments that exceed 72 hours have been excluded.} \label{fig:rm-memory}
\vspace{-3mm}
\end{figure}


==> revision/twitter-large.tex <==
\renewcommand{\thefigure}{A}
\begin{figure}[h]
\centering
\begin{tikzpicture}
    \begin{customlegend}[legend columns=7,
        legend entries={\cseedselect{,~}$\epsilon=\frac{1}{2}$,
        \cseedselect{,~}$\epsilon=\frac{1}{8}$, 
        \cseedselectp{,~}$\epsilon=\frac{1}{2}$,
        \cseedselectp{,~}$\epsilon=\frac{1}{8}$,
        \mgreedy,\lgreedy,\tgreedy
        }
        ,
        legend style={at={(0.45,1.05)},anchor=north,draw=none,font=\footnotesize,column sep=0.1cm}]
    \addlegendimage{line width=0.25mm,mark size=2pt,mark=square,color=Orange}
    \addlegendimage{line width=0.25mm,mark size=2pt,mark=pentagon,color=Orange}
    \addlegendimage{line width=0.25mm,mark size=2pt,mark=triangle,color=Red}
    \addlegendimage{line width=0.25mm,mark size=2pt,mark=diamond,color=Red}
    \addlegendimage{line width=0.25mm,mark size=2pt,mark=o, color=LightBlue}
    \addlegendimage{line width=0.25mm,mark size=2pt,mark=+, color=Green}
    \addlegendimage{line width=0.25mm,mark size=2pt,mark=x,color=DeepBlue}
    \end{customlegend}
\end{tikzpicture}
\\[-\lineskip]
\hspace{-3mm}\subfloat[\rim]{
\begin{tikzpicture}[scale=1]
    \begin{axis}[
        height=(\columnwidth/1.95)/2.8,
        width=(\columnwidth/1.95)/2.25,
        ylabel={total revenue ($\times 10^7$)},
        xlabel={$\#$RR sets},
        xmin=0, xmax=8,
        ymin=4000000, ymax=16000000,
        xtick={0, 2, 4, 6, 8},
        xticklabel style = {font=\footnotesize},
        xticklabels={$2^5$, $2^9$, $2^{13}$, $2^{17}$, $2^{21}$},
        ytick={4000000,8000000, 16000000},
        yticklabels={4, 8, 16},
        ymode=log,
        log basis y={10},
        every axis y label/.style={at={(current axis.north west)},right=10.7mm,above=0mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
        every axis x label/.style={at={(current axis.south)},right=0mm,above=-7mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
    ]

    \addplot[line width=0.2mm,mark size=2.0pt,mark=x,color=DeepBlue]
        plot coordinates { % Tgreedy
        (0, 235890.463)
        (1, 646026.087)
        (2, 1529469.886)
        (3, 2873170.825)
        (4, 4244501.078)
        (5, 5317046.000)
        (6, 6429715.904) 
        (7, 7488932.113)
        (8, 8619790.158)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=o, color=LightBlue]
        plot coordinates { % Greedy
        (0, 4378898.940)
        (1, 4793755.151)
        (2, 5479489.697)
        (3, 6726696.304)
        (4, 7942941.420)
        (5, 8892612.264)
        (6, 9891016.217)
        (7, 10837771.405) 
        (8, 11794661.969)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=+, color=Green]
        plot coordinates { % Local-Greedy
        (0, 4380009.666)
        (1, 4738357.685)
        (2, 5201947.005)
        (3, 6264773.074)
        (4, 7550438.573)
        (5, 8643948.451)
        (6, 9754396.903) 
        (7, 10839854.017)
        (8, 11897681.818)
    };
    
    \addplot[line width=0.2mm,mark size=2.0pt,mark=square,color=Orange]
        plot coordinates { % GANS-2
        (0, 5150853.603)
        (1, 6973416.347)
        (2, 8126627.755)
        (3, 9371335.228)
        (4, 10397368.493)
        (5, 11370225.745)
        (6, 12140653.160) 
        (7, 12779598.368)
        (8, 13318578.224)
    };
        
    \addplot[line width=0.2mm,mark size=2.0pt,mark=pentagon,color=Orange]
        plot coordinates { % GANS-8
        (0, 5150853.603)
        (1,  6986189.697)
        (2, 8118991.512)
        (3, 9363698.986)
        (4, 10429440.710)
        (5, 11329823.082)
        (6, 12137737.504) 
        (7, 12743777.450)
        (8, 13277342.516)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=triangle,color=Red]
        plot coordinates { % GANS-PM-2
        (0, 5150853.603)
        (1, 6992992.895)
        (2, 8191188.711)
        (3, 9373278.998)
        (4, 10413612.863)
        (5, 11335654.395)
        (6, 12099972.815) 
        (7, 12762798.635)
        (8, 13267762.503)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=diamond,color=Red]
        plot coordinates { % GANS-PM-8
        (0, 5150853.603)
        (1, 7007293.494)
        (2, 8203267.858)
        (3, 9388134.960)
        (4, 10422220.991)
        (5, 11334543.668)
        (6, 12100944.700) 
        (7, 12724339.743)
        (8, 13273454.975)
    };
    
    \end{axis}
\end{tikzpicture}\vspace{1mm}\hspace{1mm}%
}%
\hspace{-3mm}\subfloat[\mrim]{
\begin{tikzpicture}[scale=1]
    \begin{axis}[
        height=(\columnwidth/1.95)/2.8,
        width=(\columnwidth/1.95)/2.25,
        ylabel={total spread ($\times 10^6$)},
        xlabel={$\#$RR sets},
        xmin=0, xmax=8,
        ymin=5650000, ymax=45200000,
        xtick={0, 2, 4, 6, 8},
        xticklabel style = {font=\footnotesize},
        xticklabels={$2^{1}$, $2^5$, $2^9$, $2^{13}$, $2^{17}$},
        ytick={8000000, 16000000, 32000000},
        yticklabels={8, 16, 32},
        ymode=log,
        log basis y={10},
        every axis y label/.style={at={(current axis.north west)},right=10mm,above=0mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
        every axis x label/.style={at={(current axis.south)},right=0mm,above=-7mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
    ]

    \addplot[line width=0.2mm,mark size=2.0pt,mark=x,color=DeepBlue]
        plot coordinates { % Tgreedy
        (0, 607706.036)
        (1, 1776884.132)
        (2, 5316490.637)
        (3, 13990567.535)
        (4, 21768704.965)
        (5, 28053193.427)
        (6, 31739832.305) 
        (7, 33358854.485)
        (8, 34186067.773)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=o, color=LightBlue]
        plot coordinates { % Greedy
        (0, 7140858.311)
        (1, 10563422.050)
        (2, 13513649.501)
        (3, 18231181.071)
        (4, 25152115.608)
        (5, 29803003.610)
        (6, 31941845.620)
        (7, 33345525.771) 
        (8, 34170239.925)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=+, color=Green]
        plot coordinates { % Local-Greedy
        (0, 3729540.674)
        (1, 6531069.664)
        (2, 12707262.328)
        (3, 14572032.666)
        (4, 18748085.245)
        (5, 25413691.612)
        (6, 31422442.312) 
        (7, 33859097.767)
        (8, 34353093.215)
    };
    
    \addplot[line width=0.2mm,mark size=2.0pt,mark=square,color=Orange]
        plot coordinates { % GANS-2
        (0, 8522879.303)
        (1, 18496922.298)
        (2, 28448889.612)
        (3, 32844032.922)
        (4, 33149760.290)
        (5, 33341777.070)
        (6, 33008975.753) 
        (7, 33552120.832)
        (8, 34166491.224)
    };
        
    \addplot[line width=0.2mm,mark size=2.0pt,mark=pentagon,color=Orange]
        plot coordinates { % GANS-8
        (0, 8522879.303)
        (1, 18496922.298)
        (2, 28481378.352)
        (3, 32918590.414)
        (4, 33712065.395)
        (5, 34113176.370)
        (6, 33197660.355) 
        (7, 33661249.675)
        (8, 34225637.391)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=triangle,color=Red]
        plot coordinates { % GANS-PM-2
        (0, 7758144.360)
        (1, 18207855.822)
        (2, 28278948.514)
        (3, 31576555.563)
        (4, 32769891.953)
        (5, 33457570.270)
        (6, 32826122.463) 
        (7, 33697070.592)
        (8, 34266456.576)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=diamond,color=Red]
        plot coordinates { % GANS-PM-8
        (0, 7758144.360)
        (1, 18206606.255)
        (2, 27968222.878)
        (3, 32552467.312)
        (4, 33768295.906)
        (5, 34088185.032)
        (6, 33138097.666) 
        (7, 33662082.719)
        (8, 34243131.328)
    };
    
    \end{axis}
\end{tikzpicture}\vspace{1mm}\hspace{1mm}%
}%
\hspace{-3mm}\subfloat[\advim]{
\begin{tikzpicture}[scale=1]
    \begin{axis}[
        height=(\columnwidth/1.95)/2.8,
        width=(\columnwidth/1.95)/2.25,
        ylabel={reduction ($\times 10^5$)},
        xlabel={$\#$RR sets},
        xmin=0, xmax=8,
        ymin=80000, ymax=2500000,
        xtick={0, 2, 4, 6, 8},
        xticklabel style = {font=\footnotesize},
        xticklabels={$2^{1}$, $2^5$, $2^9$, $2^{13}$, $2^{17}$},
        ytick={100000, 500000, 2500000},
        yticklabels={1,5,25},
        ymode=log,
        log basis y={10},
        every axis y label/.style={at={(current axis.north west)},right=9mm,above=0mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
        every axis x label/.style={at={(current axis.south)},right=0mm,above=-7mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
    ]

    \addplot[line width=0.2mm,mark size=2.0pt,mark=x,color=DeepBlue]
        plot coordinates { % Tgreedy
        (0, 44553.685)
        (1, 90613.301)
        (2, 397720.313)
        (3, 817830.092)
        (4, 1239683.919)
        (5, 1612549.930)
        (6, 1821282.303) 
        (7, 1893650.668)
        (8, 1927077.194)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=o, color=LightBlue]
        plot coordinates { % Greedy
        (0, 86089.072)
        (1, 130855.132)
        (2, 430252.290)
        (3, 835283.449)
        (4, 1239786.889)
        (5, 1612549.930)
        (6, 1821282.303)
        (7, 1893650.668) 
        (8, 1927077.194)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=+, color=Green]
        plot coordinates { % Local-Greedy
        (0, 86089.072)
        (1, 130855.132)
        (2, 430252.290)
        (3, 835283.449)
        (4, 1239786.889)
        (5, 1612549.930)
        (6, 1821275.868) 
        (7, 1893650.668)
        (8, 1927038.580)
    };
    
    \addplot[line width=0.2mm,mark size=2.0pt,mark=square,color=Orange]
        plot coordinates { % GANS-2
        (0, 185268.161)
        (1, 400262.377)
        (2, 1037309.923)
        (3, 1351264.417)
        (4, 1660314.982)
        (5, 1803873.995)
        (6, 1884319.042) 
        (7, 1914456.975)
        (8, 1924728.198)
    };
        
    \addplot[line width=0.2mm,mark size=2.0pt,mark=pentagon,color=Orange]
        plot coordinates { % GANS-8
        (0, 185268.161)
        (1, 400262.377)
        (2, 1037309.923)
        (3, 1351264.417)
        (4, 1705248.367)
        (5, 1842654.943)
        (6, 1882278.956) 
        (7, 1894358.584)
        (8, 1897421.931)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=triangle,color=Red]
        plot coordinates { % GANS-PM-2
        (0, 185268.161)
        (1, 400262.377)
        (2, 1037618.832)
        (3, 1344088.719)
        (4, 1613766.260)
        (5, 1808263.077)
        (6, 1884949.731) 
        (7, 1914585.687)
        (8, 1924618.793)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=diamond,color=Red]
        plot coordinates { % GANS-PM-8
        (0, 185268.161)
        (1, 400262.377)
        (2, 1037618.832)
        (3, 1345948.609)
        (4, 1707179.048)
        (5, 1843182.663)
        (6, 1882195.293) 
        (7, 1894410.069)
        (8, 1897428.367)
    };
    
    \end{axis}
\end{tikzpicture}\vspace{1mm}\hspace{1mm}%
}%
\hspace{-3mm}\subfloat[\im]{
\begin{tikzpicture}[scale=1]
    \begin{axis}[
        height=(\columnwidth/1.95)/2.8,
        width=(\columnwidth/1.95)/2.25,
        ylabel={spread ($\times 10^6$)},
        xlabel={$\#$RR sets},
        xmin=0, xmax=8,
        ymin=2000000, ymax=18000000,
        xtick={0, 2, 4, 6, 8},
        xticklabel style = {font=\footnotesize},
        xticklabels={$2^{1}$, $2^5$, $2^9$, $2^{13}$, $2^{17}$},
        ytick={2000000, 4000000, 8000000, 16000000},
        yticklabels={2,4,8,16},
        ymode=log,
        log basis y={10},
        every axis y label/.style={at={(current axis.north west)},right=7.5mm,above=0mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
        every axis x label/.style={at={(current axis.south)},right=0mm,above=-7mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
    ]

    \addplot[line width=0.2mm,mark size=2.0pt,mark=x,color=DeepBlue]
        plot coordinates { % Tgreedy
        (0, 134203.485)
        (1, 745075.090)
        (2, 1714239.178)
        (3, 4113907.453)
        (4, 7314381.501)
        (5, 11152301.278)
        (6, 13951247.830)
        (7, 15541030.144) 
        (8, 16263363.117)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=+, color=Green]
        plot coordinates { % Greedy
        (0, 2100938.481)
        (1, 2295121.177)
        (2, 2920904.281)
        (3, 4750520.136)
        (4, 7594950.923)
        (5, 11177126.007)
        (6, 13951247.830)
        (7, 15541030.144) 
        (8, 16263363.117)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=triangle,color=Red]
        plot coordinates { % GANS-PM-2
        (0, 2167831.963)
        (1, 3978121.183)
        (2, 7214582.758)
        (3, 10842408.687)
        (4, 12520743.642)
        (5, 13487825.119)
        (6, 14710734.591) 
        (7, 15883244.866)
        (8, 16288604.368)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=diamond,color=Red]
        plot coordinates { % GANS-PM-8
        (0, 2167831.963)
        (1, 3978121.183)
        (2, 7214582.758)
        (3, 10842408.687)
        (4, 12554232.035)
        (5, 14220404.540)
        (6, 14725812.699) 
        (7, 15926313.272)
        (8, 16312012.922)
    };
    
    \end{axis}
\end{tikzpicture}\vspace{1mm}\hspace{1mm}%
}%
\vspace{-3mm}
\caption{Result quality of element selection algorithms on Twitter-large.} 
\label{fig:result-tw}
\vspace{-2mm}
\end{figure}


==> revision/twitter-scale-large.tex <==
\renewcommand{\thefigure}{B}
\begin{figure}[h]
\centering
\begin{tikzpicture}
    \begin{customlegend}[legend columns=4,
        legend entries={\cseedselect{,~}$\epsilon=1/2$,
        \cseedselect{,~}$\epsilon=1/8$,        \cseedselectp{,~}$\epsilon=1/2$,
        \cseedselectp{,~}$\epsilon=1/8$
        }
        ,
        legend style={at={(0.45,1.05)},anchor=north,draw=none,font=\footnotesize,column sep=0.1cm}]
    \addlegendimage{line width=0.25mm,mark size=2pt,mark=square,color=Orange}
    \addlegendimage{line width=0.25mm,mark size=2pt,mark=pentagon,color=Orange}
    \addlegendimage{line width=0.25mm,mark size=2pt,mark=triangle,color=Red}
    \addlegendimage{line width=0.25mm,mark size=2pt,mark=diamond,color=Red}
    \end{customlegend}
    \begin{customlegend}[legend columns=4,
        legend entries={
    \mgreedy,\lgreedy,\tgreedy,{RR set generation}
        }
        ,
        legend style={at={(0.45,0.7)},anchor=north, draw=none,font=\footnotesize,column sep=0.1cm}]
    \addlegendimage{line width=0.25mm,mark size=2pt,mark=o, color=LightBlue}
    \addlegendimage{line width=0.25mm,mark size=2pt,mark=+, color=Green}
    \addlegendimage{line width=0.25mm,mark size=2pt,mark=x,color=DeepBlue}
    \addlegendimage{line width=0.25mm,mark size=1.5pt,mark=oplus*}
    \end{customlegend}
\end{tikzpicture}
\vspace{-2mm}
\\[-\lineskip]
\begin{tikzpicture}[scale=1]
    \begin{axis}[
        height=(\columnwidth/1.95)/2.8,
        width=(\columnwidth/1.95)/2.25,
        ylabel={running time (s)},
        xlabel={$\#$RR sets},
        xmin=0, xmax=8,
        ymin=50, ymax=100000,
        xtick={0, 2, 4, 6, 8},
        xticklabel style = {font=\footnotesize},
        xticklabels={$2^5$, $2^9$, $2^{13}$, $2^{17}$, $2^{21}$},
        ytick={100,1000,10000,100000},
        yticklabels={$10^2$,$10^3$,$10^4$,$10^5$},
        ymode=log,
        log basis y={10},
        every axis y label/.style={at={(current axis.north west)},right=8.5mm,above=0mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
        every axis x label/.style={at={(current axis.south)},right=0mm,above=-7mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
    ]

    \addplot[line width=0.2mm,mark size=1.0pt,mark=oplus*]
        plot coordinates { % RR set
        (1, 3.976)
        (2, 14.963)
        (3, 51.647)
        (4, 206.656)
        (5, 830.020)
        (6, 3348.854) 
        (7, 13366.603)
        (8, 53357.785)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=x,color=DeepBlue]
        plot coordinates { % Tgreedy
        (0, 2497.203)
        (1, 2494.615)
        (2, 2494.318)
        (3, 2494.387)
        (4, 2494.976)
        (5, 2493.959)
        (6, 2494.959)
        (7, 2491.959) 
        (8, 2483.674)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=+, color=Green]
        plot coordinates { % Greedy
        (0, 722.970)
        (1, 723.024)
        (2, 723.398)
        (3, 724.261)
        (4, 725.991)
        (5, 730.564)
        (6, 742.604)
        (7, 772.857) 
        (8, 845.987)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=+, color=Green]
        plot coordinates { % Local-Greedy
        (0, 66.605)
        (1, 66.586)
        (2, 66.590)
        (3, 66.580)
        (4, 66.639)
        (5, 67.001)
        (6, 68.357) 
        (7, 72.274)
        (8, 81.272)
    };
    
    \addplot[line width=0.2mm,mark size=2.0pt,mark=square,color=Orange]
        plot coordinates { % GANS-2
        (0, 1425.525)
        (1, 1415.323)
        (2, 1419.672)
        (3, 1429.607)
        (4, 1463.943)
        (5, 1537.440)
        (6, 1670.015) 
        (7, 1823.417)
        (8, 2015.156)
    };
        
    \addplot[line width=0.2mm,mark size=2.0pt,mark=pentagon,color=Orange]
        plot coordinates { % GANS-8
        (0, 5544.184)
        (1, 5557.069)
        (2, 5573.725)
        (3, 5619.776)
        (4, 5787.104)
        (5, 6147.343)
        (6, 6853.047) 
        (7, 7605.110)
        (8, 8308.354)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=triangle,color=Red]
        plot coordinates { % GANS-PM-2
        (0, 119.829)
        (1, 119.769)
        (2, 119.681)
        (3, 119.743)
        (4, 119.914)
        (5, 120.802)
        (6, 125.096) 
        (7, 133.706)
        (8, 155.117)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=diamond,color=Red]
        plot coordinates { % GANS-PM-8
        (0, 438.970)
        (1, 438.527)
        (2, 438.504)
        (3, 438.624)
        (4, 441.043)
        (5, 442.529)
        (6, 454.838) 
        (7, 489.643)
        (8, 571.539)
    };
    
    \end{axis}
\end{tikzpicture}
\vspace{-4mm}
\caption{Running time of element selection algorithms in \rim on Twitter-large.} \label{fig:tw-rm-time}
\vspace{-3mm}
\end{figure}

\vspace{-5mm}

\renewcommand{\thefigure}{C}
\begin{figure}[h]
\centering
\begin{tikzpicture}
    \begin{customlegend}[legend columns=2,
        legend entries={\ouralgo, \rma
        }
        ,
        legend style={at={(0.51,2.35)},draw=none,font=\footnotesize,column sep=0.1cm}]
    \addlegendimage{line width=0.25mm,mark size=2pt,mark=triangle,color=Red}
    \addlegendimage{line width=0.25mm,mark size=2pt,mark=pentagon,color=Pink}
    \end{customlegend}
\end{tikzpicture}
\vspace{-2mm}
\\[-\lineskip]
\begin{tikzpicture}[scale=1]
    \begin{axis}[
        height=(\columnwidth/1.95)/2.8,
        width=(\columnwidth/1.95)/2.25,
        ylabel={running time (s)},
        xlabel={approx. guarantee},
        xmin=0, xmax=0.6,
        ymin=100, ymax=312000,
        xtick={0,0.2, 0.4,0.6},
        xticklabel style = {font=\footnotesize},
        xticklabels={0,0.2, 0.4,0.6},
        ytick={100, 1000, 10000, 100000},
        yticklabels={$10^2$, $10^3$, $10^4$, $10^5$},
        ymode=log,
        log basis y={10},
        every axis y label/.style={at={(current axis.north west)},right=8.5mm,above=0mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
        every axis x label/.style={at={(current axis.south)},right=0mm,above=-7mm},
        label style={font=\footnotesize},
        tick label style={font=\footnotesize},
    ]


    \addplot[line width=0.2mm,mark size=2.0pt,mark=pentagon,color=Pink]
        plot coordinates { 
        (0,513.603)
        (0.1, 2087.931)
        % (0.2,3.490)
        % (0.3,13.252)
        % (0.4,101.423)
    };

    \addplot[line width=0.2mm,mark size=2.0pt,mark=triangle,color=Red]
        plot coordinates { % ours
        (0.13212+0, 175.318)
        (0.13212+0.1, 517.097)
        (0.13212+0.2, 234613.649)
        % (0.13212+0.3, 16.120)
        % (0.13212+0.4, 35.460)
    };
    
    \end{axis}
\end{tikzpicture}
\vspace{-4mm}
\caption{Running time of scalable algorithms in \rim on Twitter-large. Experiments that exceed 72 hours have been excluded.} \label{fig:tw-rm-scale-time}
\vspace{-4mm}
\end{figure}

==> sec/exp.tex <==




\input{fig/fig-rm-spread}
\input{fig/fig-mrim-spread}
\input{fig/fig-advim-spread}

\section{Experiments}\label{sec:exp}
We first introduce the experimental settings in \S~\ref{sec:exp-setting}, and then evaluate the performance of our proposal in \S~\ref{sec:exp-performance}. All experiments are conducted on a Linux machine with Intel Xeon(R) Gold 6240@2.60GHz CPU and 377GB RAM in single-thread mode. \eat{As a preview, in our experiments, the case consuming the most memory (Figure~\ref{fig:scale-rm-time}(f)) occupies no more than 30\% of the total memory.}


\subsection{Experimental Setups}\label{sec:exp-setting}

\stitle{Datasets}
\edit{We experiment with \revise{7} real-world datasets that are widely adopted in previous works and publicly available at SNAP~\cite{snapnets}: Facebook~\cite{zhu2020pricing,li2018automated,becker2021influence}, Wiki~\cite{li2018automated}, Twitter~\cite{becker2021influence}, Google+~\cite{zhu2020pricing}, Pokec~\cite{tang2018online}, LiveJournal~\cite{tang2018online,zhu2020pricing}, \revise{and Twitter-large~\cite{tang2018online}. The largest Twitter-large dataset is the largest dataset ever used in instances \rim, \mrim, and \advim, with 41.7 million nodes and 1.5 billion edges.}
The dataset statistics are listed in Table~\ref{tab:dataset}.
% In addition, previous instances of \ourproblem were evaluated on the graph with at most xxx edges~\cite{xxx}. In contrast, this work includes the LiveJournal graph containing tens of millions of edges. 
}

\begin{table}[!t]
\centering
\caption{Dataset statistics. ($K=10^3, M=10^6, B=10^9$)}\label{tab:dataset}
\vspace{-3mm}
\renewcommand{\arraystretch}{1.2}
\begin{footnotesize}
\begin{tabular}{ccccc}
\toprule
\textbf{Name}     & \textbf{\#nodes} & \textbf{\#edges} & \revise{\textbf{Type}} & \revise{\textbf{Avg. degree}} \\ 
% \textbf{Name}     & Facebook & Wiki & Twitter & Google+ & Pokec & LiveJournal \\ 
\midrule 
Facebook & $4.0K$ & $176.4K$ & \revise{friendship} & \revise{$43.6$}\\
Wiki & $7.1K$ & $103.6K$ & \revise{who-votes-on-whom} & \revise{$14.5$}\\
Twitter & $81.3K$ & $1.7M$ & \revise{who-follows-whom} & \revise{$21.7$}\\
Google+ & $107.6K$ & $13.7M$ & \revise{who-follows-whom} & \revise{$283.3$}\\
Pokec & $1.6M$ & $30.6M$ & \revise{friendship} & \revise{$18.7$}\\
LiveJournal & $4.8M$ & $69.0M$ & \revise{friendship} & \revise{$14.2$}\\
Twitter-large & $41.7M$ & $1.5B$ & \revise{who-follows-whom} & \revise{$35.2$}\\
\bottomrule
\end{tabular}
\end{footnotesize}
\vspace{-1mm}
\end{table}

\stitle{\ourproblem instances and configurations}
We focus on the instances \im, \rim, \mrim, and \advim, as illustrated in \edit{\S~\ref{sec:imgm}-\ref{sec:imgm-instance}.} Following the default configurations in \yiqiann{related works}~\cite{han2021efficient, sun2018multi, sun2023scalable, guo2020influence}, we use the \ic model in \rim, \mrim, \im and the \lt model in \advim. We set $p_{i,j}=1/|N^{in}_j|$ for all $e_{i,j}\in E$. \eat{In addition, }We configure $T=10,\alpha_i = 1,k_j=1$ for all $i\in [T],v_j\in V$ for \rim, set $T=20,k=100$ for \mrim, and $k=2000$ for \im. In the absence of a ground-truth set $A$ for \advim, where $|A|$ represents \shiqi{the number of contagious seeds} \eat{the existing spread }as detected by the authority, we generate a synthetic set $A$. This is accomplished by initially adding the node $v_i$\eat{, which has the largest out-degree,} with the largest out-degree to set $A$. Following this, each out-neighbor $v_j$ of $v_i$ is independently added to $A$ with a probability of $p_{i,j}$. Furthermore, we set $k_v=500$ and $k_e=1000$, which are comparable in magnitude to $|A|$.


\stitle{Algorithms and constant settings} 
We evaluate the performance of 9 algorithms in total, which are divided into two parts: 5 algorithms for \edit{element} selection, and 4 algorithms for their scalable implementation. These algorithms are as follows.
\begin{itemize}[topsep=2pt,itemsep=1pt,parsep=0pt,partopsep=0pt,leftmargin=11pt]
    \item \textit{\edit{Element} selection}: \shiqi{\mgreedy, \lgreedy, and \tgreedy (baselines in \S~\ref{sec:existing}); \cseedselect and \cseedselectp for the general matroid and partition matroid, respectively (Algorithm~\ref{alg:greedy-framework}).}
    \item \textit{Scalable solutions}: \shiqi{\rma for \rim~\cite{han2021efficient}, \naimm for \mrim~\cite{sun2018multi}, and \advimm for \advim~\cite{sun2023scalable} (baselines); \ouralgo (Algorithm~\ref{alg:ouralgo}).}
\end{itemize}
For all \edit{element} selection algorithms, we apply the lazy evaluation technique in \cite{minoux1978accelerated,leskovec2007cost} to improve their empirical efficiency.
For \cseedselect and \cseedselectp, $\epsilon$ is set to $1/2$ and $1/8$. Based on Theorem~\ref{thm:gans-correct}, these settings provide an approximation of 0.56 and 0.61 for \eat{the RR set coverage function}\yiqiann{maximizing} $\Lambda_{\R}$, respectively, \shiqi{indicating a focus on efficiency but at the cost of result quality, and vice versa.} For \tgreedy, $\xi$ is set to {the default value} $0.05$~\cite{bian2020efficient}. 
For all scalable implementations, we set $\delta=1/|V|$ by default and vary $\epsilon$ from 0.5 to 0.1~\cite{tang2018online,tang2015influence}. For a fair comparison, we have also made other necessary modifications to scalable competitors and refer interested readers to \trref{\ref{sec:exp-detail}} for details. In addition, for each algorithm, we estimate the objective function value $\sigma$ by averaging over $10,000$ Monte Carlo simulations. We repeat each algorithm 5 times and report the average when evaluating the running time and the objective function value. All algorithms are implemented in C++ with \texttt{-O3} optimization\eat{, available at: {\color{blue}\url{https://anonymous.4open.science/r/IMGM-920B/}}}.

\input{fig/rm-time}

\input{fig/fig-im-spread}


\input{fig/scale-rm-time}
% \input{fig/scale-rm-rrset}
\input{fig/scale-other-time}
% \input{fig/scale-other-rrset}

\vspace{-1mm}
\subsection{Performance Evaluations}\label{sec:exp-performance}

\stitle{Performance of \edit{element} selection in \rim, \mrim, and \advim}
In the first set of experiments, we evaluate the result quality and running time of \edit{element} selection algorithms on the \ourproblem instances \rim, \mrim, and \advim. For a fair comparison, we provide all algorithms with the same \LL{collection of RR sets $\R$}. Furthermore, we vary $|\R|$ from $2^5$ to $2^{21}$ in \rim; and from $2^1$ to $2^{17}$ in \mrim and \advim. \shiqi{The choices of the smallest and largest values for $|\R|$ roughly correspond to $\theta_{1}$ and $\theta_{max}$ in Algorithm~\ref{alg:ouralgo} when $\epsilon=0.1$.}

\noindent
\textit{Result quality.} As shown in Figures~\ref{fig:rm-spread}-\ref{fig:advim-spread}, both \cseedselect and \cseedselectp return better solutions compared to their competitors in terms of related objective functions across all datasets. For instance,  \cseedselect or \cseedselectp outperforms all competitors by up to $86\%$ on Pokec in \rim, $708\%$ on Wiki in \mrim, \revise{$205.8\%$ on Twitter-large} in \advim.
To explain, \cgreedy and \cgreedyp select each element based on the largest partial derivative and subsequently update the value of $q_R$ for each $R$ containing the selected element. In contrast to the competitors \mgreedy, \lgreedy, and \tgreedy, \shiqi{our} update strategy circumvents the direct exclusion of each related $R$ and offers a more fine-grained marginal coverage for each element. As a result, it allows for a more refined and potentially more effective selection process.
Furthermore, we observe that the result quality of \tgreedy is much worse than other approaches when the number of RR sets is small. This is because it disregards all elements whose marginal coverage is below the minimum threshold, rendering the number of selected elements fewer than expected.



% \stitle{Running time}
\noindent 
\textit{Running time.} In the second set of experiments, we use \rim as the instance and report the running times of \edit{element} selection algorithms in Figure~\ref{fig:rm-time}. Similar trends were observed in the running time results for other instances. Specifically, \lgreedy and \cseedselectp (with $\epsilon=1/2$) are the fastest and second-fastest algorithms respectively, across all datasets, each being $4-10\times$ faster than \mgreedy. Recall from the first set of experiments that \lgreedy, despite being the fastest, is the second least effective algorithm, quality wise. Furthermore, \shiqi{we compare \cseedselect and \cseedselectp with the same $\epsilon$ values across these problems using partition matroids. In particular, }\cseedselectp improves the running time by an order of magnitude. These observations demonstrate the efficiency of \cseedselectp, as proved in \S~\ref{sec:put-together}. Note that, in Figure~\ref{fig:rm-time}(e), the running time of \cseedselect decreases when $|\R|\geq 2^{15}$, due to the lazy evaluation technique. 
We also report the time taken to generate $\R$. RR set generation becomes more expensive than all \edit{element} selection methods as the size of $\R$ increases. For instance, when $|\R|> 2^9$ on Facebook, the time taken to generate $\R$ exceeds that of \cseedselectp by more than an order of magnitude. %Specifically, the cost of RR set generation becomes overwhelming if a large number of redundant RR sets are generated. 
This motivates the design of an efficient scheme for RR set generation, as proposed in \S~\ref{sec:opimc}. 

\input{fig/fig-rm-memory-formal}
\input{fig/fig-other-memory}

\noindent 
\textbf{Performance of \edit{element} selection in \im.}
In the third set of experiments, we evaluate the performance of the proposed \edit{element} selection methods on the conventional \im problem. Here, we only compare \cseedselect with \mgreedy and \tgreedy as \cseedselect and \cseedselectp (resp. \mgreedy and \lgreedy) are \LL{essentially equivalent.} Figure~\ref{fig:im-spread} reports the spread of each method on different datasets \edit{as} $|\R|$ is varied from $2^1$ to $2^{17}$. Notably, \shiqi{\cseedselect outperforms competitors by up to $871\%$ on LiveJournal. This is attributed to the more fine-grained marginal coverage, as discussed earlier.}

\noindent 
\textbf{Effect of $\epsilon$ in \cseedselect.}
Next, we examine the impact of the $\epsilon$ parameter in the proposed \cseedselect algorithm. Here, we focus on the result qualities of \cseedselect and \mgreedy, as shown in Figures~\ref{fig:rm-spread}-\ref{fig:im-spread}. Note that \cseedselect is equivalent to \mgreedy when $\epsilon=1$. Based on observations in the first and third sets of experiments, the result quality of \cseedselect improves significantly by decreasing $\epsilon$ from $1$ to $1/2$ (\ie increasing the number of iterations in Line 4 of Algorithm~\ref{alg:greedy-framework} from 1 to 2). This improvement becomes less pronounced with further increases in the number of iterations. For example, in \mrim, the solution quality of \cseedselect improves by $84\%$ on Pokec when $|\R|=2^9$ as $\epsilon$ decreases from $1$ to $1/2$. In contrast, the improvement is only $7\%$ when comparing $\epsilon=1/2$ with $\epsilon=1/8$.
% the result qualities of 4 variants of our proposal, \cseedselect and \cseedselectp with $\epsilon=1/2$ and $\epsilon=1/8$, differ by less than $3\%$ in most cases;



% \subsection{Performance of \ouralgo}\label{sec:exp-opim}
\stitle{Performance of scalable implementations}
Finally, we evaluate the running times \revise{and memory usages} of \ouralgo and all scalable competitors by varying $\epsilon$ from $0.5$ to $0.1$. In \revise{Figures~\ref{fig:scale-rm-time}-\ref{fig:scale-other-memory}}, the approximation \yiqiann{ratio} of each solution is used as the x-axis, with \ouralgo having $1-1/e-\epsilon$ and all competitors having $1/2-\epsilon$.

\noindent
\textit{Running time.}
Figure \ref{fig:scale-rm-time} reports the running time for each solution in \rim; \LL{in Figure~\ref{fig:scale-rm-time}(g), we exclude approaches that run more than 72 hours.} Specifically, \ouralgo consistently outperforms \rma in terms of running time while ensuring the same approximation guarantee across all cases. Notably, \ouralgo is an order of magnitude faster than \rma on Google+, Pokec, and LiveJournal.
\revise{In addition, \ouralgo completes within 66 hours on Twitter-large  when $\epsilon=0.3$, whereas \rma only returns results for $\epsilon\geq 0.4$ and fails to terminate even after 7 days when $\epsilon=0.3$.}
Figure~\ref{fig:scale-other-time} presents similar outcomes for \mrim and \advim on Facebook and Wiki. Here, \ouralgo is at least three orders of magnitude faster than \naimm in \mrim and at least two orders faster than \advimm in \advim. Note that we exclude results on other datasets as \naimm and \advimm fail to terminate within 72 hours even when $\epsilon=0.5$.
The reason for the efficiency of \ouralgo is twofold. First, \ouralgo introduces the early termination and the tightened bound \edit{$\Lambda^u_{\R_1}(S^*)$}, which allows us to generate an appropriate number of RR sets as soon as a $(1-1/e-\epsilon)$-approximation is reached. Furthermore, \cseedselect provides superior result qualities during iterations, \LL{enabling \ouralgo to reach the desired approximation faster.} In contrast, \rma, \naimm, and \advimm generate a large number of RR sets and reply on \mgreedy or \lgreedy for \edit{element} selection, leading to inferior result qualities. \shiqi{To summarize, the proposed \ouralgo is significantly faster than all competitors while providing the same result quality.}

\revise{
\noindent
\textit{Memory usage.}
We report the memory usage of each scalable implementation for \rim, \mrim, or \advim at its peak memory consumption in Figures \ref{fig:memory-formal}-\ref{fig:scale-other-memory}.
As shown, the memory usage of each algorithm is roughly proportional to its running time reported in Figures \ref{fig:scale-rm-time}-\ref{fig:scale-other-time}. Most notably, the memory occupancy of \ouralgo is consistently lower than that of \rma, \naimm, and \advimm due to the smaller number of sampled RR sets. Specifically, the memory footprint of \ouralgo in \mrim is at least an order of magnitude lower than \naimm on Facebook and Wiki. Note that, \ouralgo or \rma has a memory footprint of 102GB on Twitter-large when $\epsilon \geq 0.4$. Of this, 62GB is allocated for storing the dataset (with half for the original graph and half for the reversed graph, on which the RR sets are generated), while the remaining 40 GB ($\sim$39\%) is used for storing the sampled RR sets. In conclusion, the resource utilization of the proposed \ouralgo is superior to all competitors.
}


% We also report the running time of \ouralgo with $\epsilon=0.1$ on larger datasets in Table~\ref{tab:time-scalable-others}, which demonstrates the scalability of our proposal. Note that \naimm and \advimm fail to terminate within 24 hours on larger datasets.

% \begin{table}[!t]
% \centering
% \renewcommand{\arraystretch}{1.2}
% \caption{Running time of \ouralgo with $\epsilon=0.1$ on larger datasets, in seconds.}\vspace{-2mm}
% \begin{small}
% % \resizebox{\columnwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% \textbf{Problem}   & Twitter     & Google+  & Pokec  & Orkut  \\ \hline
% \mrim   & \hl{running} & \hl{running} & \hl{running} & \hl{running} \\ \hline
% \advim   & 70.605     & 2813.481  & 1351.196  & 7689.379  \\ \hline
% \end{tabular}
% % }
% \end{small}\label{tab:time-scalable-others}
% \vspace{-2mm}
% \end{table}
